On the multiplicative independence between $n$ and $\lfloor \alpha n\rfloor$

In this article we investigate different forms of multiplicative independence between the sequences $n$ and $\lfloor n \alpha \rfloor$ for irrational $\alpha$. Our main theorem shows that for a large class of arithmetic functions $a, b \colon \mathbb{N} \to \mathbb{C}$ the sequences $(a(n))_{n \in \mathbb{N}}$ and $(b ( \lfloor \alpha n \rfloor))_{n \in \mathbb{N}}$ are asymptotically uncorrelated. This new theorem is then applied to prove a $2$-dimensional version of the Erd\H{o}s-Kac theorem, asserting that the sequences $(\omega(n))_{n \in \mathbb{N}}$ and $(\omega( \lfloor \alpha n \rfloor)_{n\in \mathbb{N}}$ behave as independent normally distributed random variables with mean $\log\log n$ and standard deviation $\sqrt{ \log \log n}$. Our main result also implies a variation on Chowla's Conjecture asserting that the logarithmic average of $(\lambda(n) \lambda ( \lfloor \alpha n \rfloor))_{n \in \mathbb{N}}$ tends to $0$.

==> dumpedproofs.tex <==

%This is the proof for Van der Corput
%\begin{proof}
%    We want to show that $\forall \epsilon > 0$
%    \begin{center}
%        $\limsup\limits_{N \rightarrow \infty} |\frac{1}{N} \sum\limits_{n=1}^{N} u_n| < \epsilon$
%    \end{center}
%    Notice that for any $\epsilon > 0$ and any $D \in \mathbb{N}$, if $N \in \mathbb{N}$ is large enough we have
%    \begin{center}
%        $|\frac{1}{N} \sum\limits_{n=1}^N u_n - \frac{1}{ND}\sum\limits_{n=1}^N \sum\limits_{d=1}^D u_{n+d}| < \frac{\epsilon}{2}$
%    \end{center}
%    Meaning it suffices to show that, if $D$ is large enough,
%    \begin{center}
%        $\limsup\limits_{N \rightarrow \infty}|\frac{1}{ND} \sum\limits_{n=1}^N \sum\limits_{d=1}^D u_{n+d}| < \frac{\epsilon}{2}$
%    \end{center}
%    Thus, using Cauchy-Schwarz inequality we get 
%    \begin{equation}
%        \limsup\limits_{N \rightarrow \infty} |\frac{1}{ND} \sum\limits_{n=1}^N \sum\limits_{d=1}^D u_{n+d}|^2 \leq \frac{1}{D^2} \sum\limits_{d_1, d_2 = 1}^D \limsup\limits_{N \rightarrow \infty} \frac{1}{N} \sum\limits_{n=1}^N u_{n+d_1} \overline{u_{n+d_2}}
%    \end{equation}
%    Notice that for $d_1 \neq d_2$, it follows from the hypothesis that $\frac{1}{N} \sum_{n=1}^N u_{n+d_1}\overline{u_{n+d_2}} \rightarrow 0$ as $N \rightarrow \infty$. We conclude that expression (2.3) is bounded by $\frac{D}{D^2} = \frac{1}{D}$, which gets arbitrarily small as $D \rightarrow \infty$.
%\end{proof}

%\begin{Lemma}[\Katai{}-Criterion]
%    Let $f : \N \to \C$ bounded. If for all primes $p \neq q$ such that :
%    \begin{align*}
%        \frac{1}{N} \sum_{n=1}^N  f(pn) \overline{f(qn)} \to 0
%    \end{align*}
%    then 
%    \begin{align*}
%        \frac{1}{N} \sum_{n=1}^N f(n) \to 0
%    \end{align*}
%\end{Lemma}


---PROOF OF 1.16---

\begin{proof}
\begin{align*}
    |a(pn)b(qn)- \theta_p^a\theta_q^ba(n)b(n)| &\leq |a(pn)b(qn)-\theta_p^a a(n) b(qn)|+|\theta_p^a a(n) b(qn)- \theta_p^a\theta_q^ba(n)b(n)|\\
    &\leq ||b||_\infty|a(pn)-\theta_p^aa(n)|+ ||a||_\infty||(\theta_p^a)_p||_\infty |b(pn) -\theta_q^bb(n)|\\
    &=o_p(1)+o_q(1),
\end{align*}
which gives
$$\limsup_N| a(pn)b(pn)- \theta_p^a\theta_p^ba(n)b(n)|\leq ||b||_\infty o_p(1)+ ||a||_\infty||(\theta_p^a)_p||_\infty o_q(1)=o_p(1)+o_q(1).$$
\end{proof}

\begin{Proposition}
Let $a,b:\N\to \C$ BMAI sequences. Then $a\cdot b:=(a(n)b(n))_n$ is BMAI.
\end{Proposition}
\begin{proof}
The fact that $a\cdot b$ is bounded is direct, and the second condition comes from Proposition \ref{BMAItwoprimes} with $p=q$. Note that $(\theta_p^2)_{p\in \mathcal{P}}$ is the corresponding sequence of $\theta$'s.
\end{proof}
